Fast Flow Volume Estimation

The increasing popularity of jumbo frames means growing variance in the size of packets transmitted in modern networks. Consequently, network monitoring tools must maintain explicit traffic volume statistics rather than settle for packet counting as before. We present constant time algorithms for volume estimations in streams and sliding windows, which are faster than previous work. Our solutions are formally analyzed and are extensively evaluated over multiple real-world packet traces as well as synthetic ones. For streams, we demonstrate a run-time improvement of up to 2.4X compared to the state of the art. On sliding windows, we exhibit a memory reduction of over 100X on all traces and an asymptotic runtime improvement to a constant. Finally, we apply our approach to hierarchical heavy hitters and achieve an empirical 2.4-7X speedup.

==> TopK.tex <==
\subsection{Top-k Identification}

\begin{figure*}[t!]
	\begin{tabular}{ccc}
		\subfloat[CAIDA]{\label{top512Caida}\includegraphics[width = \matrixCellWidth]
			{topKPlots/512-from-1024/Caida-avgConvergence--512-using-1024.pdf}} &
		\subfloat[UCLA]{\label{top512UCLA}\includegraphics[width = \matrixCellWidth]
			{topKPlots/512-from-1024/UCLA-avgConvergence--512-using-1024.pdf}} &
		\subfloat[YouTube]{\label{top512YouTube}\includegraphics[width = \matrixCellWidth]
			{topKPlots/512-from-1024/Youtube-avgConvergence--512-using-1024.pdf}}\\
		\subfloat[Zipf0.6]{\label{top512Zipf06}\includegraphics[width = \matrixCellWidth]
			{topKPlots/512-from-1024/Zipf06-avgConvergence--512-using-1024.pdf}} &
		\subfloat[Legend]{\includegraphics[width = 4cm]
			{TopKLegend.png}}&		
		\subfloat[Zipf0.8]{\label{top512Zipf08}\includegraphics[width = \matrixCellWidth]
			{topKPlots/512-from-1024/Zipf08-avgConvergence--512-using-1024.pdf}} \\
		\subfloat[Zipf1.0]{\label{top512Zipf10}\includegraphics[width = \matrixCellWidth]
			{topKPlots/512-from-1024/Zipf10-avgConvergence--512-using-1024.pdf}} &
		\subfloat[Zipf1.2]{\label{top512Zipf12}\includegraphics[width = \matrixCellWidth]
			{topKPlots/512-from-1024/Zipf12-avgConvergence--512-using-1024.pdf}} &
		\subfloat[Zipf1.5]{\label{top512Zipf15}\includegraphics[width = \matrixCellWidth]
			{topKPlots/512-from-1024/Zipf15-avgConvergence--512-using-1024.pdf}}
	\end{tabular}
\caption{\label{top512}The average recall achieved for identifying the top-$512$ using 1024 counters, compared to the size of the stream. }
\end{figure*}


\begin{figure*}[t]
	\begin{tabular}{ccc}
		\subfloat[CAIDA]{\label{top512tradeoffCaida}\includegraphics[width = \matrixCellWidth]
			{topKPlots/512-from-1024/Caida-avgCurves-512-using-1024.pdf}} &
		\subfloat[UCLA]{\label{top512tradeoffUCLA}\includegraphics[width = \matrixCellWidth]
			{topKPlots/512-from-1024/UCLA-avgCurves-512-using-1024.pdf}} &
		\subfloat[YouTube]{\label{top512tradeoffYouTube}\includegraphics[width = \matrixCellWidth]
			{topKPlots/512-from-1024/Youtube-avgCurves-512-using-1024.pdf}}\\
		\subfloat[Zipf0.6]{\label{top512tradeoffZipf06}\includegraphics[width = \matrixCellWidth]
			{topKPlots/512-from-1024/Zipf06-avgCurves-512-using-1024.pdf}} &
		\subfloat[Legend]{\includegraphics[width = 4cm]
			{TopKLegend.png}}&		
		\subfloat[Zipf0.8]{\label{top512tradeoffZipf08}\includegraphics[width = \matrixCellWidth]
			{topKPlots/512-from-1024/Zipf08-avgCurves-512-using-1024.pdf}} \\
		\subfloat[Zipf1.0]{\label{top512tradeoffZipf10}\includegraphics[width = \matrixCellWidth]
			{topKPlots/512-from-1024/Zipf10-avgCurves-512-using-1024.pdf}} &
		\subfloat[Zipf1.2]{\label{top512tradeoffZipf12}\includegraphics[width = \matrixCellWidth]
			{topKPlots/512-from-1024/Zipf12-avgCurves-512-using-1024.pdf}} &
		\subfloat[Zipf1.5]{\label{top512tradeoffZipf15}\includegraphics[width = \matrixCellWidth]
			{topKPlots/512-from-1024/Zipf15-avgCurves-512-using-1024.pdf}}
	\end{tabular}
	\caption{\label{top512tradeoff}The Precision-Recall curves for identifying the top-$512$ with 1024 counters. }
\end{figure*}

Since, CS and CMS do not solve the top-$k$ problem, we only compare PSS and 16W-PSS to SS and FR.
In some of the figures we also gave PSS half the number of counters as the rest.
That configuration is marked as 0.5-PSS.

\paragraph{Top-32}
Our first test case is identifying the top-$32$ flows.
We measure the relation between the number of counters and the obtained recall.
Our results are summarized in Figure~\ref{fig:top32}, demonstrating that 16W-PSS is almost as accurate as PSS in all workloads.

Figure~\ref{top32Caida} presents results for CAIDA.
As shown, PSS and 16W-PSS achieve near perfect recall with 128 counters.
In contrast, FR and SS require 1024 counters for the same recall.
Results for UCLA are in Figure~\ref{top32UCLA}.
As can  be seen, PSS and 16W-PSS reach near optimal recall with 128 counters while FR and SS require 256 counters.

Figure~\ref{top32YouTube} shows that in the YouTube workload, 1024 counters are not enough for SS and FR, and they reach less than 0.5 recall with 1024 counters.
In comparison, PSS and 16W-PSS reach near perfect recall with 512 counters.

We now use synthetic Zipf distributions to characterize the performance envelope of PSS and 16W-PSS.
Figure~\ref{top32Zipf06} shows that for the mildly skewed Zipf 0.6, both PSS and 16W-PSS achieve near optimal recall with 256 counters while for the alternatives even 2048 are not enough.
In the somewhat more skewed Zipf 0.8 distribution, Figure~\ref{top32Zipf08} shows that PSS requires 64 counters, and 16W-PSS requires 128 to achieve near perfect recall. In contrast, SS and FR require 1024 counters~to~do~the~same.

For Zipf 1.0 distribution, Figure~\ref{fig:Zipf1.0MSE} shows that PSS and 16W-PSS still require 64 and 128 counters to achieve near optimal recall.
FR and SS now require 512 counters to do the same.
In Zipf 1.2 distribution, Figure~\ref{fig:Zipf1.2MSE} shows that PSS and 16W-PSS continue to require 64 and 128 counters, while SS and FR now require 256 counters to achieve near optimal recall.
Finally, for the very skewed Zipf 1.5, Figure~\ref{fig:Zipf1.5MSE} shows that PSS and 16W-PSS still require 64 and 128 counters to achieve near optimal recall while SS and FR now require 128 counters.
To sum it up, PSS shows a reduction of 2x-16x that depending how workload skeweness.
% requires 64 counters and 16W-PSS 128 counters. In this workload tough, the alternatives also require 128 counters to identify the top 32. However, even in these conditions PSS requires half as many counters and 16W-PSS converges better than the alternatives.

\paragraph{Top-512 with 1024 counters}
Our next test case is evaluating top-512 flows with 1024 counters.
This time, we focus on how stable the recall rates are during the workloads.
Note that the top-512 items also change during the trace and the algorithms are required to constantly adjust.
To quantify the improvement of PSS in these settings we use 0.5-PSS, which attempts to identify the top-512 with mere 512 counters.
Our results are illustrated in Figure~\ref{top512}.
As can be seen, PSS and 16W-PSS offer similar recall rates in all the tested workloads.

Figure~\ref{top512Caida} exhibits the results for CAIDA workload.
As shown, PSS, 16W-PSS and even 0.5-PSS are significantly better than SS and FR.
In Figure~\ref{top512UCLA}, we see that in the UCLA workload, PSS and 16W-PSS achieve around 97\% recall while SS and FR achieve less than 92\%.
Interestingly, in this trace, even 0.5-PSS is above 90\% recall with just 512 counters.

Figure~\ref{top512YouTube} shows results for the difficult YouTube trace.
%As can be seen, the YouTube workload is significantly more difficult.
Yet, PSS and 16W-PSS achieve above 50\% recall, while SS and FR are constantly under 20\% recall.
The improvement is more than x2, as 0.5 PSS is significantly better than FR and SS.

We now use synthetic workloads to identify the performance envelope of PSS and 16W-PSS.
We can observe that as the workload becomes more skewed, all the algorithms improve but PSS and 16W-PSS remain considerably better than the alternatives.
For the mildly skewed Zipf 0.6 distribution, Figure~\ref{top512Zipf06} shows that PSS and 16W-PSS achieve over 50\% recall while FR and SS are under 10\%.
In the slightly more skewed Zipf 0.8, Figure~\ref{top512Zipf08} exhibits that PSS and 16W-PSS yield over 90\% recall, while the alternatives are slightly below 20\%. Similarly, in Zipf 1.0, Figure~\ref{top512Zipf10} shows that  PSS and 16W PSS are  close to 100\% recall during the entire trace while SS and FR are only at 40\% recall.
In  Zipf 1.2, Figure~\ref{top512Zipf12} shows that SS and FR reach 60\% while PSS and 16W-PSS remain at 100\%.
Finally for Zipf 1.5, Figure~\ref{top512Zipf15} shows that SS and FR are approaching 85\% recall.
Even in this workload, 0.5-PSS eventually achieves higher recall.
In all these cases, 0.5-PSS achieves higher recall than SS and FR and the space reduction is at least x2.

\paragraph{Precision and recall trade-off}
%Recall is not everything, as there is also the question of precision.
While recall is an important measure of the algorithms success, when more than $k$ items are reported as suspected top-$k$, the precision is compromised.
Returning all the items yields the maximum recall, but also poor precision when many items are monitored. The ideal behavior of a top-$k$ algorithm is 100\% precision and 100\% recall (the top right position in the graphs).
Figure~\ref{top512tradeoff} illustrates the precision and recall trade-off.
For each recall level, we measure how many elements were returned to achieve it, and compute the corresponding precision. %the maximum precision that satisfies it. %Note that the only variable is, how many entries are returned.

Figures~\ref{top512tradeoffCaida} shows our results for the CAIDA workload.
As can be seen, PSS and 16W-PSS perform the best on this workload as they can provide 80\% recall with near 100\% precision, or $\approx 90\%$ recall with $\approx 90\%$ precision.
At the same time, their maximum recall is close to 100\%, but returning all items drops precision to 50\%.
SS and FR perform worse as their maximum recall is 60\% and they can only grantee 30\% recall with high precision.

Figure~\ref{top512tradeoffUCLA} shows results for the UCLA workload.
As can be seen, PSS and 16W-PSS offer the best precision and recall trade-off, although in this case SS and FR also perform well.

Figure~\ref{top512tradeoffYouTube} shows results for the YouTube workload.
As can be observed, this trace is significantly more difficult.
PSS and 16W-PSS perform better than the rest.
Their maximal recall is slightly over 60\% but over 50\% recall is possible with very high precision.
SS and FR achieves less than 20\% maximal recall and very poor precision.

We now look into what happens in synthetic traces.
For Zipf 0.6 distribution, Figure~\ref{top512tradeoffZipf06} shows that PSS and 16W-PSS can achieve over 50\% recall with good accuracy, while SS and FR achieve less than 10\% recall.
In the slightly more skewed Zipf 0.8, Figure~\ref{top512tradeoffZipf08} shows that PSS and 16W PSS perform very well
%are already near optimal
.
They can offer $\approx 90\%$ recall and precision.
SS and FR improve slightly, both offer bad accuracy but the maximum recall of SS is 30\% and FR is slightly less than 20\%.
The non-monotone rise in the SS curve is explained by coincidentally having higher rates of top-$512$ elements in the lower estimated frequency counters.
For Zipf 1.0, 1.2 and 1.5, Figure~\ref{top512tradeoffZipf10}, Figure~\ref{top512tradeoffZipf12} and Figure~\ref{top512tradeoffZipf15} show that while PSS and 16W-PSS provides near optimal precision and recall, SS and FR gradually improve as the skew increases.
They achieve $\approx 50\%$ recall at Zipf 1.0, $\approx 70\%$ recall at Zipf 1.2 and slightly over 80\% recall with high precision with Zipf 1.5.
However, in all these cases, 0.5 PSS is better than FR and SS and thus the space reduction is more than x2 across the entire range.

%In this case, 0.5 PSS is still slightly better than the rest and PSS and 16W-PSS offers almost the ideal recall and precision ration.

%but in that trace the alternatives are also good. Still, PSS and 16W-PSS out perform the rest.
%In Figure~\ref{top512tradeoffYouTube}, we can see that for the YouTube trace, the overall recall is lower, yet over 0.5 recall can be achieved with maximal precision for both PSS and 16W-PSS. In this case the alternatives yield very poor precision and recall.
%From the rest synthetic traces in Figures~\ref{top512tradeoffZipf06}, (Zipf 0.6), Figure~\ref{top512tradeoffZipf08} (Zipf 0.8) Figure~\ref{top512tradeoffZipf10} (Zipf 1.0), Figure~\ref{top512tradeoffZipf12} and Figure~\ref{top512tradeoffZipf15} (Zipf 1.5), we can see when the distribution becomes more skewed identifying the top-k becomes easier. PSS and 16W PSS provide very high precision and recall from Zipf 0.8 onwards, and the alternatives improves as the workload becomes more skewed. Yet, even for Zipf 1.5, PSS and 16W-PSS offer a superior precision/recall trade-off than the rest.

% shows the precision and recall trade-off for the Caida trace. In this trace the performance of a fully associative and 16-Way PSS are the best followed by Space Saving and half memory PSS. SpaceSaving seems to be doing better on the UCLA trace, but it is only marginally more accurate then 0.5 PSS. Thus the improvement in accuracy is very significant. In this trace, PSS and 16W- PSS identify over 95\% of the top 512 with very high precision, and their maximum recall is 100\%.

%Figure~\ref{fig:UCLARecallTop512} provides us with additional insight about the maximum recall throughout the trace. As can be seen in the early stages SpaceSavings was very accurate, but as the trace progresses its recall drops as the top items become more difficult to identify. The graph of space savings intersects that of 0.5 PSS, multiple times, and the two seem to converge to similar maximum recall despite the fact that 0.5 PSS only has 512 counters to identify top 512 flows.

%\paragraph{YouTube Trace~\cite{YouTube}}


%Figure~\ref{fig:YouTubeTop512} shows results on the YouTube trace. At first glance it appears that the YouTube trace is a lot more difficult then both the UCLA and Caida traces. As it is probably less skewed. As can be seen, PSS is able to identify 50\% of the top 512 with high precision and its maximum recall is almost 70\%. 16W-PSS lags a bit behind due to associativity problems but it is still significantly better then a fully associative PSS with half as many counters (0.5 PSS). SpaceSavings and Frequent perform very poorly and their maximum recall is less then 20\%. We therefore repeated the YouTube trace with the more modest ambition of identifying the top 128 flows with 1024 counters. The results are reported in Figure~\ref{fig:YouTubeTop128}, as can be observed SpaceSaving and Frequent do not provide a reasonable result even with these conditions. On the contrary, all 3 of our PSS variants achieve over 80\% max recall. Moreover, PSS and 16W-PSS are able to get over 80\% recall with over 90\% accuracy.

%\paragraph{Synthetic Zipf Traces}
%We continue our evaluation to characterize the performance of PSS in identifying top-k under various conditions with different Zipf conditions. Figure~\ref{fig:Zipf01Top512} shows accuracy and recall of identifying top 512 on Zipf 1.0 and Figure~\ref{fig:Zipf06Top512} on Zipf 0.6. As can be observed, in both conditions, PSS and its variants are significantly better than the alternatives, even when PSS is given only half as many counters.




==> TopKV2.tex <==



%\begin{figure*}[t]
%	\begin{tabular}{ccc}
%		\subfloat[Caida]{\includegraphics[width = \matrixCellWidth]
%			{topKPlots/128-from-1024/Caida-Convergence--128-using-1024.pdf}} &
%		\subfloat[UCLA]{\includegraphics[width = \matrixCellWidth]
%			{topKPlots/128-from-1024/UCLA-Convergence--128-using-1024.pdf}} &
%		\subfloat[YouTube]{\includegraphics[width = \matrixCellWidth]
%			{topKPlots/128-from-1024/Youtube-Convergence--128-using-1024.pdf}}\\
%		\subfloat[Zipf0.6]{\includegraphics[width = \matrixCellWidth]
%			{topKPlots/128-from-1024/Zipf06-Convergence--128-using-1024.pdf}} &
%		\subfloat[Legend]{\includegraphics[width = 5.5cm]
%			{TopKLegend.png}}&		
%		\subfloat[Zipf0.8]{\includegraphics[width = \matrixCellWidth]
%			{topKPlots/128-from-1024/Zipf08-Convergence--128-using-1024.pdf}} \\
%		\subfloat[Zipf1.0]{\includegraphics[width = \matrixCellWidth]
%			{topKPlots/128-from-1024/Zipf10-Convergence--128-using-1024.pdf}} &
%		\subfloat[Zipf1.2]{\includegraphics[width = \matrixCellWidth]
%			{topKPlots/128-from-1024/Zipf12-Convergence--128-using-1024.pdf}} &
%		\subfloat[Zipf1.5]{\includegraphics[width = \matrixCellWidth]
%			{topKPlots/128-from-1024/Zipf15-Convergence--128-using-1024.pdf}} 
%		
%	\end{tabular}
%	\caption{The recall for finding the top-32 elements vs. number of counters.}
%\end{figure*}






==> conclusions.tex <==
\section{Conclusion and Discussion}
In this paper, we have presented Probabilistic Space Saving (PSS), a novel algorithm for approximate frequency estimation and top-$k$ identification.
We have also introduced $d$-Way Probabilistic Space Saving ($d$W-PSS), a hardware friendly variant of PSS.
We have extensively evaluated PSS and $d$W-PSS for both problems under two packet traces and a YouTube video trace as well as multiple synthetic Zipf like traces.
These experiments exhibited significant reductions in the memory requirements of PSS and $d$W-PSS compared to state of the art alternatives for obtaining the same error.
In top-$k$, we showed that our algorithms achieve superior precision/recall than the alternatives in any tested situation.
In the case of frequency estimation, the only exception is the highly skewed UCLA trace~\cite{UCLA}, and even there, it is only when all schemes are allocated a very large number of counters compared to the trace.
Notice that in that specific case, all algorithms yield a very precise estimation since with so many counters on such a skewed trace, the problem becomes almost trivial.

In contrast, PSS and $d$W-PSS are the only algorithms that performed well on heavy-tailed distributions, which are common in Internet based services.

Another benefit of PSS and $d$W-PSS is that they incur fewer updates to memory since they do not replace a counter with each untracked item.
This is especially true in heavy-tailed workloads.
We have not included the evaluation and quantification of this property for lack of space.

Since $d$W-PSS can be implemented as a simple cache policy, in the future we would like to integrate it into real networking devices.
Interestingly, we believe that $d$W-PSS may also offer benefits for software implementations.
For example, it can probably be parallelized efficiently since each operation only computes the minimum over a small fixed set of counters.


==> evaluation.tex <==
\section{Evaluation}
\label{sec:results}
In this section, we evaluate PSS and $d$W-PSS along with the following previously suggested algorithms -- Frequent(\emph{FR})~\cite{BatchDecrement} and Space-Saving(\emph{SS})~\cite{SpaceSavings}.
These counter-based algorithms were proven effective for both frequency and top-$k$ estimation.
In particular, Space Saving is considered the state of the art~\cite{SpaceSavingIsTheBest}.
For frequency estimation, we also compare our approach with sketches such as Count-Sketch~(\emph{CS})~\cite{CountSketch} and Count-Min-Sketch (\emph{CMS})\cite{CountMinSketch}.

For equal number of counters, frequency sketches are asymptotically worse than counter based algorithms.
However, they do not maintain a flow to counter association and thus require less memory per counter.

For a fair comparison, we evaluate the performance of CS and CMS using 8 times as many counters as the rest of the (counter based) algorithms.
They were configured to use 4 lines, which was shown effective in practice~\cite{caffein}.
By giving the sketches more counters, we compensate for their lower overheads, as they do not maintain a flow to counter association and avoid storing flow identifiers.
%This is done to reflect possible additional overheads from maintaining flow to counter association and storing flow identifiers by counter based algorithms.
We consider this a generous comparison, as the flow id and metadata overheads should not take more than $7$ times the counter size.


\subsection{Datasets}
Our evaluation includes the following datasets:
\begin{enumerate}
	\item The CAIDA Anonymized Internet Trace 2015 \cite{CAIDA} , or in short \emph{CAIDA}. The data is collected from the `equinix-chicago' high-speed monitor and contains 18M elements of mixed UDP, TCP and ICMP packets.
	\item The UCLA Computer Science department packet trace (denoted \emph{UCLA})\cite{UCLA}. This trace contains 32M UDP packets passed through the border router of the CS Department, University of California, Los Angeles.
	\item YouTube Trace from the UMass campus network (referred to as \emph{YouTube})~\cite{youtube}. The trace includes a sequence of 600K accesses to YouTube from within the university.
	\item Zipf streams. Self-generated traces of identical and independently distributed elements sampled from a Zipf distribution with various skew values ($0.6, 0.8, 1.0, 1.2$ and $1.5$).
	Hereafter, the skew $X$ stream is denoted~Zipf$X$.
%	The stream with skew $X$ is heretofore denoted as \emph{Zipf$X$}.
\end{enumerate}

\subsection{Metrics}
%Our evaluation discusses two problems with the following performance metrics:
Our evaluation considers the following performance metrics:
\begin{enumerate}
\item \textbf{On-Arrival frequency estimation} \\
Many networking applications take decisions on a \emph{per-packet} basis.
For example, if a router identifies excessive traffic originating from a specific source, the router may suspend further routing of its packets to prevent denial of service attacks.
We refer to this as the \emph{On-Arrival} model, where upon arrival of each packet, the algorithms are required to estimate its flow frequency.
Formally, a stream $S=s_1,s_2,\ldots$ is revealed one element at a time; upon arrival of item $s_t$, an algorithm \emph{Alg} is required to provide an estimate $\widehat{f_{s_t}}$ for the number elements in the stream with the same id. We then measure the \emph{Mean Square Error} (MSE) of the algorithm, i.e.,
$$MSE(Alg) = \frac{1}{N}\sum_{t=1}^{N}(\widehat{f_{s_t}} - f_{s_t})^2.$$

\item \textbf{Top-$k$ Identification} \\
The ability to identify the most frequent flows is also important to many applications.
We define the \emph{Top-$k$} identification problem as follows: 
Given a stream $S=s_1,s_2,\ldots$ and two query parameters $m$ and $k$, the algorithm is required to output a set of $m$ elements containing as many of the $k$ most frequent stream elements as possible.
We denote the $k$-highest element frequency by $F_k$.
For a set of candidates $C$, we measure its quality using the standard recall and precision metrics:
\begin{align*}
&\text{Precision}(C) &=\ \  &|e\in C : f_e \ge F_k| / |C|\\
&\text{Recall}(C)    &=\ \  &|e\in C : f_e \ge F_k| / k
\end{align*}
%We also define the \textbf{\emph{$k$-Accuracy}} measure, which evaluates how many of elements from the top-$k$ the algorithm is able to identify with a set {\bf of size $k$} (note that this quantity also equals the precision \emph{and} recall of the returned set).
%we consider the problem of approximating the frequency of an arriving element, a
\end{enumerate}

\input{onArrival}
\input{TopK}


==> side-by-side-algs.tex <==
\begin{algorithm*}%[H]
	\begin{tabular}{c|c}
		\begin{minipage}{0.45\textwidth}
			\begin{algorithmic}[1]
				\State $c_x = c_x + 1$
			\end{algorithmic}
%			\caption{Alg A}
\captionof{algorithm}{Your caption}
			\label{alg:a}							
		\end{minipage}
		&
		\begin{minipage}{0.45\textwidth}	
			\begin{algorithmic}[1]
				\State $c_x = c_m + 1$	
			\end{algorithmic}
%			\caption{Alg B}
		\captionof{algorithm}{Your caption}
			\label{alg:b}
		\end{minipage}
	\end{tabular}
\end{algorithm*}


%\begin{algorithm*}%[H]
%%	\begin{minipage}{0.45\textwidth}
%%		\rule{\linewidth}{2cm}
%\begin{tabular}{c|c}
%	\begin{minipage}{0.45\textwidth}
%		Initialization: $C=\emptyset, \forall i: c_i=0, \forall i: \varepsilon_i=0$
%		\begin{algorithmic}[1]
%			\Function{Add}{Item $x$}
%			\If {$x\in C$}
%			\State $c_x = c_x + 1$
%			\Else\If {$|C| < M$}
%			\State $c_x = 1$
%			\State $C = C \cup \{x\}$
%			\Else
%			\State $m = \text{argmin}_{y\in C} c_y$
%			\State $C = C \setminus \{m\} \cup \{x\}$
%			\State $c_x = c_m +1$
%			\State $\varepsilon_x = m$
%			\EndIf\EndIf
%			\EndFunction
%			\captionof{figure}{Some figure}
%
%		\end{algorithmic}
%			\caption{Space-Saving}
%			\label{alg:SpaceSaving}							
%
%	\end{minipage}
%	&
%	\begin{minipage}{0.45\textwidth}	
%	Initialization: $C=\emptyset, \forall i: c_i=0$
%	\begin{algorithmic}[1]
%		\Function{Add}{Item $x$}
%		\If {$x\in C$}
%		\State  $c_x= c_x+1$
%		\Else\If {$|C| < M$}
%		\State $c_x = 1$
%		\State $C = C \cup \{x\}$
%		\Else
%		\State $m = \text{argmin}_{y\in C} c_y$
%		\If {$random()<{\left(\frac{1}{c_m+1}\right)}$}
%		\State $C = (C \setminus \{m\}) \cup \{x\}$
%		\State $c_x = c_m + 1$
%		\EndIf\EndIf\EndIf
%		\EndFunction
%	\caption{Probabilistic Space Saving}		
%	\end{algorithmic}
%
%	\label{alg:PSS}
%
%	\end{minipage}\\
%		
%\end{tabular}
%
%\end{algorithm*}


%
%\begin{algorithm}[h]
%	\begin{minipage}{0.45\textwidth}
%	Initialization: $C=\emptyset, \forall i: c_i=0$
%	\begin{algorithmic}[1]
%		\Function{Add}{Item $x$}
%		\If {$x\in C$}
%		\State  $c_x= c_x+1$
%		\Else\If {$|C| < M$}
%		\State $c_x = 1$
%		\State $C = C \cup \{x\}$
%		\Else
%		\State $m = \text{argmin}_{y\in C} c_y$
%		\If {$random()<{\left(\frac{1}{c_m+1}\right)}$}
%		\State $C = (C \setminus \{m\}) \cup \{x\}$
%		\State $c_x = c_m + 1$
%		\EndIf\EndIf\EndIf
%		\EndFunction
%	\end{algorithmic}
%	\caption{Probabilistic Space Saving}
%	\label{alg:PSS}
%\end{minipage}	
%\end{algorithm}
%\begin{algorithm*}%[H]
%	\begin{minipage}{0.45\textwidth}
%		\rule{\linewidth}{2cm}
%		\begin{algorithm}[h]
%			\begin{minipage}{0.45\textwidth}
%				Initialization: $C=\emptyset, \forall i: c_i=0, \forall i: \varepsilon_i=0$
%				\begin{algorithmic}[1]
%					\Function{Add}{Item $x$}
%					\If {$x\in C$}
%					\State $c_x = c_x + 1$
%					\Else\If {$|C| < M$}
%					\State $c_x = 1$
%					\State $C = C \cup \{x\}$
%					\Else
%					\State $m = \text{argmin}_{y\in C} c_y$
%					\State $C = C \setminus \{m\} \cup \{x\}$
%					\State $c_x = c_m +1$
%					\State $\varepsilon_x = m$
%					\EndIf\EndIf
%					\EndFunction
%				\end{algorithmic}
%				\caption{Space-Saving}
%				\label{alg:SpaceSaving}
%			\end{minipage}\hfill
%		\end{algorithm}
%		\caption{left side of a pretty pretty long long
%			long very very long caption}
%	\end{minipage}\hfill
%	\begin{minipage}{0.45\textwidth}
%		\rule{\linewidth}{4cm}
%		\caption{right side of a pretty pretty long long
%			long very very long caption}
%	\end{minipage}
%\end{algorithm*}
%
%\begin{figure*}
%	\makeatletter
%	\def\@captype{algocf}
%	\makeatother
%	\begin{minipage}{0.45\textwidth}
%		\rule{.5\linewidth}{2cm}
%	\end{minipage}\hfill
%	\begin{minipage}{0.45\textwidth}
%		\rule{\linewidth}{4cm}
%	\end{minipage}
%\end{figure*}

==> sliwi_comparison_table.tex <==

\newcommand{\tabColWidth}{1.33cm}

\begin{table}[tp]
	\tiny
	\begin{tabular}{|p{0.9cm}|@{}p{\tabColWidth}|@{}p{\tabColWidth}|@{}p{\tabColWidth}|p{0.9cm}|p{0.45cm}|}
		\hline
		& Memory Requirement & \quad{}Update Time   			& \heavyHitters{} Query Time	& \windowcounting{} Query Time	 & Static Memory\\ \hline
		Arasu and Manku~\cite{ArasuM04}&
		$\begin{aligned}
		O\parentheses{\oneOverE\log^2\oneOverE}
		\end{aligned}$
		& $\begin{aligned}
			O\parentheses{\oneOverE\log\oneOverE}
		\end{aligned}$ &
		$\begin{aligned}
			O\parentheses{\oneOverE\log\oneOverE}
		\end{aligned}$ & N/A & \quad\xmark
		\\ \hline
		Hung and Ting \cite{LeeT06}& 		$\begin{aligned}
			O\parentheses{\oneOverE}
		\end{aligned}$
		&$\begin{aligned}
			O\parentheses{\oneOverE}
		\end{aligned}$	
		&$\begin{aligned}
			O\parentheses{\oneOverE}
		\end{aligned}$	& N/A & \quad{}\xmark
		\\ \hline
		Hung et al. \cite{HungLT10} &
		$\begin{aligned}
			O\parentheses{\oneOverE}
		\end{aligned}$			& $O(1)$
		&$\begin{aligned}
			O\parentheses{\oneOverE}
		\end{aligned}$	
		&  N/A & \quad{}\xmark
		\\ \hline
		This Paper &	$\begin{aligned}
			O\parentheses{\oneOverE}
		\end{aligned}$
		& $O(1)$ 
		&$\begin{aligned}
			O\parentheses{\oneOverE}
		\end{aligned}$	
		& {$O(1)$} & \quad{}\cmark{}
		\\ \hline		
	\end{tabular}\smallskip
	\normalsize
	\caption{Comparison of Sliding Window Algorithms. }
	\label{tab:bs}
\end{table} 

